Uncovering the Inner Workings of STEGO for Safe Unsupervised Semantic Segmentation

Self-supervised pre-training strategies have recently shown impressive results for training general-purpose feature extraction backbones in computer vision. In combination with the Vision Transformer architecture, the DINO self-distillation technique has interesting emerging properties, such as unsupervised clustering in the latent space and semantic correspondences of the produced features without using explicit human-annotated labels. The STEGO method for unsupervised semantic segmentation contrastively distills feature correspondences of a DINO-pre-trained Vision Transformer and recently set a new state of the art. However, the detailed workings of STEGO have yet to be disentangled, preventing its usage in safety-critical applications. This paper provides a deeper understanding of the STEGO architecture and training strategy by conducting studies that uncover the working mechanisms behind STEGO, reproduce and extend its experimental validation, and investigate the ability of STEGO to transfer to different datasets. Results demonstrate that the STEGO architecture can be interpreted as a semantics-preserving dimensionality reduction technique.

==> arxiv zip/table_config.tex <==
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{\vspace{-3mm}\thead{Parameter}} & \multicolumn{4}{c}{\thead{\textbf{Configuration}} } \\ \cmidrule(lr){2-5} 
                                        & \multicolumn{3}{c}{Actual} & Reported \\ 
\midrule
{Dataset} & Cocostuff & Cityscapes & Potsdam & * \\ 
{Train steps \hspace{-1mm}} & {7000} & {7000} & 5000 & - \\  % AlexK inserted hspace{-1mm} here because otherwise we had overflown hbox by 0.5mm 
{Batch size} & {32} & {32} & 16 & 32 \\ 
{Crop type} & {5-crop} & {5-crop} & No crop & 5-crop \\ 
{Backbone} & {ViT-B} & {ViT-B} & ViT-S & ViT-B \\ 
{0-clamp} & {-} & {-} & True & True \\ 
{Pointwise} & {True} & {False} & True & True \\ 
$D_\textrm{STEGO}$ & {90} & {100} & 70 & 70 \\ 
$\lambda_\textrm{rand}$ & {0.15} & {0.91} & 0.63 & * \\ 
$\lambda_\textrm{knn}$ & {1.00} & {0.58} & 0.25 & * \\ 
$\lambda_\textrm{self}$ & {0.10} & {1.00} & 0.67 & * \\ 
$b_\textrm{rand}$ & {1.00} & {0.31} & 0.76 & * \\ 
$b_\textrm{knn}$ & {0.20} & {0.18} & 0.02 & * \\ 
$b_\textrm{self}$ & {0.12} & {0.46} & 0.08 & *  \\
\bottomrule
\end{tabular}
% OLD TABLE
% \begin{tabular}{|l|lll|l|}
% \hline
%  & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Actual Configuration} \\ from pretrained models \cite{hamilton2022unsupervised}\end{tabular} } & \begin{tabular}[c]{@{}l@{}}\textbf{Reported Config.} \\ from Sec. A.10 \\and Table 5 \cite{hamilton2022unsupervised}\end{tabular} \\ \hline
% \texttt{dataset\_name} & \multicolumn{1}{l|}{cocostuff27} & \multicolumn{1}{l|}{cityscapes} & potsdam & * \\ \hline
% \texttt{max\_steps} & \multicolumn{1}{l|}{7000} & \multicolumn{1}{l|}{7000} & 5000 & - \\ \hline
% \texttt{batch\_size} & \multicolumn{1}{l|}{32} & \multicolumn{1}{l|}{32} & 16 & 32 \\ \hline
% \texttt{crop\_type} & \multicolumn{1}{l|}{five} & \multicolumn{1}{l|}{five} & no crop & five \\ \hline
% \texttt{model\_type} & \multicolumn{1}{l|}{vit\_base} & \multicolumn{1}{l|}{vit\_base} & vit\_small & vit\_base \\ \hline
% \texttt{dim}, \ie, $D_\textrm{STEGO}$ & \multicolumn{1}{l|}{90} & \multicolumn{1}{l|}{100} & 70 & 70 \\ \hline
% \texttt{zero\_clamp} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & True & True \\ \hline
% \texttt{pointwise} & \multicolumn{1}{l|}{True} & \multicolumn{1}{l|}{False} & True & True \\ \hline
% \texttt{neg\_inter\_weight}, \ie, $\lambda_\textrm{rand}$ & \multicolumn{1}{l|}{0.1538476246} & \multicolumn{1}{l|}{0.9058762625} & 0.63 & * \\ \hline
% \texttt{pos\_inter\_weight}, \ie, $\lambda_\textrm{knn}$ & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{0.5774534831} & 0.25 & * \\ \hline
% \texttt{pos\_intra\_weight}, \ie, $\lambda_\textrm{self}$ & \multicolumn{1}{l|}{0.1} & \multicolumn{1}{l|}{1} & 0.67 & * \\ \hline
% \texttt{neg\_inter\_shift}, \ie, $b_\textrm{rand}$ & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{0.3136124189} & 0.76 & * \\ \hline
% \texttt{pos\_inter\_shift}, \ie, $b_\textrm{knn}$ & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.1754346515} & 0.02 & * \\ \hline
% \texttt{pos\_intra\_shift}, \ie, $b_\textrm{self}$ & \multicolumn{1}{l|}{0.12} & \multicolumn{1}{l|}{0.4582847221} & 0.08 & * \\ \hline
% \end{tabular}

==> arxiv zip/table_config_all.tex <==
\begin{tabular}{lrrrr}
\toprule

Parameter & Value \\ 
\midrule
%{Train resolution} & {224}  \\
%{Validation resolution} & {320}  \\
%{Nearest neighbors} & {7}  \\ 
{Loader crop type} & {Center}  \\ 
{Extra clusters} & {0}  \\ 
%{DINO patch size} & {8} \\
{Optimizers} & {Adam \cite{adam2015}}  \\ 
{Linear and cluster probe learning rates} & {0.005}  \\ 
%{Cluster probe learning rate} & {0.005}  \\
{Segm. head learning rate} & {0.0005}  \\ 
{Segm. head dropout probability} & {0.1}  \\ 
{Feature samples} & {11}  \\ 
{Negative samples} & {5}  \\
\bottomrule
\end{tabular}

==> arxiv zip/table_results.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
\multirow{3}{*}{\vspace{-9mm}Method} & \multicolumn{4}{c}{\textbf{Cocostuff}} & \multicolumn{4}{c}{\textbf{Cityscapes}} & \multicolumn{4}{c}{\textbf{Potsdam}} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
  & \multicolumn{2}{c}{\thead{Unsupervised\\ Cluster probe}} & \multicolumn{2}{c}{\thead{Supervised\\ Linear probe}} 
  & \multicolumn{2}{c}{\thead{Unsupervised\\ Cluster probe}} & \multicolumn{2}{c}{\thead{Supervised\\ Linear probe}}
  & \multicolumn{2}{c}{\thead{Unsupervised\\ Cluster probe}} & \multicolumn{2}{c}{\thead{Supervised\\ Linear probe}} 
  \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
  & \thead{Acc} & \thead{mIoU} & \thead{Acc} & \thead{mIoU} & \thead{Acc} & \thead{mIoU} & \thead{Acc} & \thead{mIoU} & \thead{Acc} & \thead{mIoU} & \thead{Acc} & \thead{mIoU} \\ \midrule
STEGO (theirs)& 56.9 & {28.2} & 76.1 & 41.0 & 73.2 & {21.0} & - & - & 77.0 & {-} & - & - \\
STEGO (ours)& {\color[HTML]{13D9C1} $^\checkmark$56.9} & {{\color[HTML]{13D9C1} $^\checkmark$28.2}} & {\color[HTML]{13D9C1} $^\checkmark$76.1} & {\color[HTML]{13D9C1} $^\checkmark$41.1} & {\color[HTML]{13D9C1} $^\checkmark$73.2} & {{\color[HTML]{13D9C1} $^\checkmark$21.0}} & {89.6} & {28.0} & {\color[HTML]{13D9C1} $^\checkmark$77.0} & {{62.6}} & {85.9} & {74.8} \\
DINO (theirs)& 30.5 & {9.6} & 66.8 & 29.4 & - & {-} & - & - & - & {-} & - & - \\
DINO (ours)& { \color[HTML]{9e36ff} $^\dagger$42.4} & {{\color[HTML]{9e36ff}  $^\dagger$13.0}} & {\color[HTML]{9e36ff}  $^\dagger$75.8} & {\color[HTML]{FF5565} $^\ddagger$44.4} & 52.6 & {15.2} & {\color[HTML]{FF5565} $^\ddagger$91.3} & {\color[HTML]{FF5565} $^\ddagger$34.9} & 71.3 & {54.3} & 84.5 & 72.8 \\ 
\bottomrule
\end{tabular}
% OLD TABLE
%\begin{tabular}{|l|cccc|cccc|cccc|}
%     \hline
%     Dataset & \multicolumn{4}{c|}{\textbf{Cocostuff}} & \multicolumn{4}{c|}{\textbf{Cityscapes}} & \multicolumn{4}{c|}{\textbf{Potsdam}} \\ \hline
%     Evaluation & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Unsupervised \\Cluster Probe\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Supervised \\Linear Probe\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Unsupervised \\Cluster Probe\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Supervised \\Linear Probe\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Unsupervised \\Cluster Probe\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Supervised \\Linear Probe\end{tabular}} \\
%     \hline
%     Metric & Acc & \multicolumn{1}{c|}{mIoU} & Acc & mIoU & Acc & \multicolumn{1}{c|}{mIoU} & Acc & mIoU & Acc & \multicolumn{1}{c|}{mIoU} & Acc & mIoU \\ \hline
%     STEGO (theirs)& 56.9 & \multicolumn{1}{c|}{28.2} & 76.1 & 41.0 & 73.2 & \multicolumn{1}{c|}{21.0} & - & - & 77.0 & \multicolumn{1}{c|}{-} & - & - \\
%     STEGO (ours)& {\color[HTML]{13D9C1} 56.93} & \multicolumn{1}{c|}{{\color[HTML]{13D9C1} 28.19}} & {\color[HTML]{13D9C1} 76.13} & {\color[HTML]{13D9C1} 41.08} & {\color[HTML]{13D9C1} 73.17} & \multicolumn{1}{c|}{{\color[HTML]{13D9C1} 21.01}} & {89.64} & {27.96} & {\color[HTML]{13D9C1} 77.03} & \multicolumn{1}{c|}{{62.57}} & {85.85} & {74.83} \\
%     DINO (theirs)& 30.5 & \multicolumn{1}{c|}{9.6} & 66.8 & 29.4 & - & \multicolumn{1}{c|}{-} & - & - & - & \multicolumn{1}{c|}{-} & - & - \\
%     DINO (ours)& {\color[HTML]{9e36ff} 42.38} & \multicolumn{1}{c|}{{\color[HTML]{9e36ff} 13.02}} & {\color[HTML]{9e36ff} 75.82} & {\color[HTML]{FF5565} 44.40} & 52.60 & \multicolumn{1}{c|}{15.20} & {\color[HTML]{FF5565} 91.27} & {\color[HTML]{FF5565} 34.91} & 71.29 & \multicolumn{1}{c|}{54.28} & 84.53 & 72.75 \\ \hline
%     \end{tabular}
